(Semi-)External Algorithms for Graph Partitioning and Clustering

In this paper, we develop semi-external and external memory algorithms for graph partitioning and clustering problems. Graph partitioning and clustering are key tools for processing and analyzing large complex networks. We address both problems in the (semi-)external model by adapting the size-constrained label propagation technique. Our (semi-)external size-constrained label propagation algorithm can be used to compute graph clusterings and is a prerequisite for the (semi-)external graph partitioning algorithm. The algorithm is then used for both the coarsening and the refinement phase of a multilevel algorithm to compute graph partitions. Our algorithm is able to partition and cluster huge complex networks with billions of edges on cheap commodity machines. Experiments demonstrate that the semi-external graph partitioning algorithm is scalable and can compute high quality partitions in time that is comparable to the running time of an efficient internal memory implementation. A parallelization of the algorithm in the semi-external model further reduces running time.

==> generate_plot_rgg <==
set terminal postscript enhanced color size 7,7
set output '| ps2pdf - outputrgg31.pdf'

set logscale x 
set xrange [1:16]
set datafile separator ","
set title "rgg31" font "Times,30" offset 0,1 
set ylabel "time t [s]"  font "Times,30" offset -4,0
set xlabel "number of PEs p" font "Times,30" offset 0,-2.5
set key samplen 5 spacing 3 font ",23"
set size ratio 1
set xtics ("2^0" 1,"2^1" 2,"2^2" 4, "2^3" 8, "2^4" 16)
set xtics font "Times,30" offset 0,-1
set ytics font "Times,30" offset -.5,0

plot "data.csv" using 1:2 title "Total Time" with linespoints lw 3, \
      "data.csv" using 1:3 title "Lowerbound Total Time" with linespoints lw 3, \
      "data.csv" using 1:4 title "Time LPA" with linespoints lw 3, \
      "data.csv" using 1:5 title "Lowerbound LPA" with linespoints lw 3, \
 



==> generate_plots <==
set terminal postscript enhanced color size 7,7
set output '| ps2pdf - output.pdf'

set logscale x 
set xrange [1:16]
set datafile separator ","
set title "uk-2007" font "Times,30" offset 0,1 
set ylabel "time t [s]"  font "Times,30" offset -4,0
set xlabel "number of PEs p" font "Times,30" offset 0,-2.5
set key samplen 5 spacing 3 font ",23"
set size ratio 1
set xtics ("2^0" 1,"2^1" 2,"2^2" 4, "2^3" 8, "2^4" 16)
set xtics font "Times,30" offset 0,-1
set ytics font "Times,30" offset -.5,0

plot "data.csv" using 1:2 title "Total Time" with linespoints lw 3, \
      "data.csv" using 1:4 title "Lower Bound Total Time" with linespoints lw 3, \
      "data.csv" using 1:3 title "Time LPA" with linespoints lw 3, \
      "data.csv" using 1:5 title "Lower Bound LPA" with linespoints lw 3, \
 



==> makros.tex <==
% anderweitig wiederverwendbare Makros fuer Diss
\usepackage{amsfonts}

% allgemeine mathematische Notation
\newcommand{\ceil}[1]{\left\lceil #1\right\rceil}
\newcommand{\floor}[1]{\left\lfloor #1\right\rfloor}
\newcommand{\abs}[1]{\left| #1\right|}
\newcommand{\seq}[1]{\langle #1\rangle}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\enorm}[1]{\norm{#1}_{2}}
\newcommand{\sumnorm}[1]{\norm{#1}_{1}}
\newcommand{\maxnorm}[1]{\norm{#1}_{\infty}}
\newcommand{\xor}{\oplus}
\newcommand{\set}[1]{\left\{ #1\right\}}
\newcommand{\gilt}{:}
\newcommand{\sodass}{\,:\,}
\newcommand{\setGilt}[2]{\left\{ #1\sodass #2\right\}}
\newcommand{\Def}{:=}
\newcommand{\zvektor}[2]{\left(#1,#2\right)}
\newcommand{\vektor}[2]{\left(\begin{smallmatrix}#1\\#2\end{smallmatrix}\right)}
\newcommand{\condition}[1]{\left[#1\right]}
\newcommand{\binomial}[2]{\binom{#1}{#2}}
\newcommand{\even}{\mathrm{even}}
\newcommand{\odd}{\mathrm{odd}}
\newcommand{\mymod}{\,\bmod\,}
\newcommand{\divides}{|}

\newcommand{\blank}{\Box}
\newcommand{\cross}[2]{\langle #1,#2 \rangle}
\newcommand{\defeq}{\mathrel{:=}}
\newcommand{\hash}{\sym{@}}
\newcommand{\hD}[1][D]{^{(#1)}}
\newcommand{\hed}[1][D]{^{1/#1}}
\newcommand{\Lpal}{L_{\mathrm{pal}}}
\newcommand{\Lparity}{L_{\mathrm{parity}}}
\newcommand{\Lvv}{L_{\mathrm{vv}}}
\newcommand{\pD}[1][D]{^{[#1]}}
\newcommand{\pos}[1]{\mathbf{#1}}
\newcommand{\qs}{\mathord{\Box}}
\newcommand{\mSet}[2]{\left\{#1 \mid #2\right\}}
\newcommand{\s}{\mathord{-}}
\newcommand{\CAce}{\hbox{\mdseries\scshape CAce}}
\newcommand{\sCAce}{\s\CAce}
\newcommand{\CAcs}{\hbox{\mdseries\scshape CAcs}}
\newcommand{\sCAcs}{\s\CAcs}
\newcommand{\CAww}{\hbox{\mdseries\scshape CAww}}
\newcommand{\sCAww}{\s\CAww}
\newcommand{\sC}{\s\hbox{\scshape Chng}}
\newcommand{\sD}{\s\hbox{\scshape Diam}}
\newcommand{\sT}{\s\hbox{\scshape Time}}
\newcommand{\CA}{\hbox{\mdseries\scshape CA}}
\newcommand{\sCA}{\s\CA}
\newcommand{\ST}[1]{\langle #1\rangle}
\newcommand{\sym}[1]{\mathord{\hbox{\texttt{\upshape #1}}}}

% Typen
\newcommand{\nat}{\mathbb{N}}
\newcommand{\natnull}{\mathbb{N}_{0}}
%\newcommand{\natless}[1]{\mathbb{N}_{<#1}}
\newcommand{\natless}[1]{\mathbb{N}_{#1}}
\newcommand{\nplus}{\mathbb{N}_+}
\newcommand{\real}{\mathbb{R}}
\newcommand{\rplus}{\mathbb{R}_+}
\newcommand{\rnneg}{\mathbb{R}_*}
\newcommand{\integer}{\mathbb{Z}}
% \newcommand{\intint}[2]{\set{#1,\ldots, #2}}
\newcommand{\intint}[2]{{#1}..{#2}}
\newcommand{\realrange}[2]{\left[#1, #2\right]}
\newcommand{\realrangeo}[2]{\left(#1, #2\right)}
\newcommand{\realrangelo}[2]{\left(#1, #2\right]}
\newcommand{\realrangero}[2]{\left[#1, #2\right)}
\newcommand{\unitrange}[2]{\realrange{0}{1}}
\newcommand{\bool}{\set{0,1}}
%\newcommand{\boolean}{\mathbb{B}}
%\newcommand{\mapping}[2]{#1\rightarrow #2}
\newcommand{\mapping}[2]{{#2}^{#1}}
\newcommand{\powerset}[1]{{\cal P}\left(#1\right)}
\newcommand{\NP}{\mathbf{NP}}
\newcommand{\Bild}{\mathbf{Bild}\:}

% Typannotation
\newcommand{\withtype}[1]{\in#1}

% Wahrscheinlichkeitsrechnung
\newcommand{\prob}[1]{{\mathbf{P}}\left[#1\right]}
\newcommand{\condprob}[2]{{\mathbf{P}}\left[#1\;|\;#2\right]}
\newcommand{\condexpect}[2]{{\mathbf{E}}\left[#1\;|\;#2\right]}
\newcommand{\expect}{{\mathbf{E}}}
\newcommand{\var}{{\mathbf{Var}}}
\newcommand{\quant}[2]{\tilde{#1}_{#2}}

% asymptotische Notation
\newcommand{\whpO}[1]{\tilde{\mathrm{O}}\left( #1\right)}
\newcommand{\Oschlange}{$\tilde{\mathrm{O}}$}
\newcommand{\Ohh}[1]{\mathcal{O}\!\left( #1\right)}
\newcommand{\Oh}[1]{\mathcal{O}\!\left( #1\right)}
\newcommand{\oh}[1]{\mathrm{o}\!\left( #1\right)}
\newcommand{\Th}[1]{\Theta\!\left( #1\right)}
\newcommand{\Thsmall}[1]{\Theta( #1)}
\newcommand{\Om}[1]{\Omega\!\left( #1\right)}
\newcommand{\om}[1]{\omega\!\left( #1\right)}
\newcommand{\Oleq}{\preceq}

% local reference
\newcommand{\lref}[1]{\ref{\labelprefix:#1}}
\newcommand{\llabel}[1]{\label{\labelprefix:#1}}
\newcommand{\labelprefix}{} % later redefined using renewcommand

% Diskussion
\newcommand{\discussionsize}{\small}
\newenvironment{discussion}{\par\discussionsize}{\par}

% open issues
%\marginparwidth5cm
\marginparpush2mm
%\newcommand{\frage}[1]{\makebox[0cm]{$\bigotimes$}\marginpar{\tiny #1}}
%\newcommand{\frage}[1]{{\sf[ #1]}\marginpar{?}}
\newcommand{\frage}[1]{}

\newcommand{\mysubsubsection}[1]{\vspace{2mm}\noindent{\bf #1 }}

% punkt am ende von display math
\newcommand{\punkt}{\enspace .}

% Pseudocode Unterst\"utzung
\newenvironment{code}{\noindent%\sf%
\begin{tabbing}%
\hspace{2em}\=\hspace{2em}\=\hspace{2em}\=\hspace{2em}\=\hspace{2em}\=%
\hspace{2em}\=\hspace{2em}\=\hspace{2em}\=\hspace{2em}\=\hspace{2em}\=%
\kill}{\end{tabbing}}

% 1=pos, 2=llable, 3=caption
\newcommand{\labelcommand}{}
\newcommand{\captiontext}{}
\newsavebox{\codeparam}
\newcounter{lineNumber}
\newenvironment{disscodepos}[3]{%
\renewcommand{\labelcommand}{#2}%
\renewcommand{\captiontext}{#3}%
\sbox{\codeparam}{\parbox{\textwidth}{#3}}%
\begin{figure}[#1]\begin{center}\begin{code}\setcounter{lineNumber}{1}}{%
\end{code}\end{center}\caption{\llabel{\labelcommand}\captiontext}\end{figure}}

\newenvironment{disscode}[2]{\begin{disscodepos}{htb}{#1}{#2}}%
{\end{disscodepos}}

% code in text 
%\newcommand{\codel}[1]{{\sf #1}}
%\newcommand{\codem}[1]{\mathsf{#1}}
\newcommand{\codel}[1]{\mbox{\rm "`#1"'}}
\newcommand{\codem}[1]{\mathrm{#1}}

\newcommand{\id}{\tt}
\newcommand{\Function} {{\bf Function\ }}
\newcommand{\Procedure}{{\bf Procedure\ }}
\newcommand{\Process}{{\bf process\ }}
\newcommand{\While}    {{\bf while\ }}
\newcommand{\Repeat}   {{\bf repeat\ }}
\newcommand{\Until}    {{\bf until\ }}
\newcommand{\Loop}     {{\bf loop\ }}
\newcommand{\Exit}     {{\bf exit\ }}
\newcommand{\Goto}     {{\bf goto\ }}
\newcommand{\Do}       {{\bf do\ }}
\newcommand{\Od}       {{\bf od\ }}
\newcommand{\Dopar}       {{\bf dopar\ }}
\newcommand{\For}      {{\bf for\ }}
\newcommand{\Step}      {{\bf step\ }}
\newcommand{\Foreach}      {{\bf foreach\ }}
\newcommand{\Rof}      {{\bf rof\ }}
\newcommand{\Forall}      {{\bf forall\ }}
\newcommand{\To}       {{\bf to\ }}
\newcommand{\If}       {{\bf if\ }}
\newcommand{\Is}       {:=}
\newcommand{\Endif}    {{\bf endif\ }}
\newcommand{\Fi}       {{\bf fi\ }}
\newcommand{\Then}     {{\bf then\ }}
\newcommand{\Else}     {{\bf else\ }}
\newcommand{\Elsif}    {{\bf elsif\ }}
\newcommand{\Return}   {{\bf return\ }}
\newcommand{\Set}      {{\bf set\ }}
\newcommand{\Boolean}  {{\bf boolean\ }}
\newcommand{\Integer}  {$\integer$}
\newcommand{\True}     {{\bf true\ }}
\newcommand{\False}    {{\bf false\ }}
\newcommand{\Bitand}   {{\bf bitand\ }}
\newcommand{\Var}      {{\bf var\ }}
\newcommand{\Xor}       {{\bf\ xor\ }}
\newcommand{\Not}       {{\bf\ not\ }}
\newcommand{\Or}       {{\bf\ or\ }}
\newcommand{\Div}       {{\bf\ div\ }}
\newcommand{\Mod}       {{\bf\ mod\ }}
\newcommand{\End}       {{\bf end\ }}
\newcommand{\Endfor}       {{\bf endfor\ }}
\newcommand{\Rem}[1]   {{\bf (*~}{\rm#1}{\bf ~*)}}
% rechtsbuendiger Kommentar
%\newcommand{\RRem}[1]   {\`{$\mathbf{(*}$~ }{\rm#1}{~$\mathbf{*)}$}}
\newcommand{\RRem}[1]   {\`{\bf --\hspace{0.5mm}--~}{\rm#1}}
\newcommand{\RRemNL}[1]   {\`{\bf (*~ }{\rm#1}{\bf ~*)}%
{\tiny\arabic{lineNumber}}\stepcounter{lineNumber}}

\newcommand{\At}[1]{\left\langle#1\right\rangle}
\newcommand{\NL}{\`{\tiny\arabic{lineNumber}}\stepcounter{lineNumber}}

% Parallelverarbeitungspseudocode
\newcommand{\iProc}{i_\mathrm{PE}}

% Parameter 1=pos, 2=xsize, 3=filename, 4=llabel, 4=caption
\newcommand{\dissepslong}[5]{\begin{figure}[#1]\begin{center}%
\epsfxsize#2\leavevmode\epsfbox{#3.eps}%
\end{center}\caption{\llabel{#4}#5}\end{figure}}

\newcommand{\dissepspos}[4]{\dissepslong{#1}{#2}{\labelprefix/#3}{#3}{#4}}
\newcommand{\disseps}[3]{\dissepspos{htb}{#1}{#2}{#3}}

% Beweise
\newdimen\endofsize\endofsize=0.5em
\def\endofbeweis{~\quad\hglue\hsize minus\hsize
                 \hbox{\vrule height \endofsize width
\endofsize}\par}
% gibt es in amsmath schon
\newenvironment{myproof}{\begin{proof}}{\endofbeweis\end{proof}}
% \newcommand{\platsch}{\hglue\hsize minus\hsize}


